Let Models Speak Ciphers: Multiagent Debate through Embeddings

Discussion and debate among Large Language Models (LLMs) have gained considerable attention due to their potential to enhance the reasoning ability of LLMs. Although natural language is an obvious choice for communication due to LLM's language understanding capability, the token sampling step needed when generating natural language poses a potential risk of information loss, as it uses only one token to represent the model's belief across the entire vocabulary. In this paper, we introduce a communication regime named CIPHER (Communicative Inter-Model Protocol Through Embedding Representation) to address this issue. Specifically, we remove the token sampling step from LLMs and let them communicate their beliefs across the vocabulary through the expectation of the raw transformer output embeddings. Remarkably, by deviating from natural language, CIPHER offers an advantage of encoding a broader spectrum of information without any modification to the model weights, outperforming the state-of-the-art LLM debate methods using natural language by 0.5-5.0% across five reasoning tasks and multiple open-source LLMs of varying sizes. This showcases the superiority and robustness of embeddings as an alternative "language" for communication among LLMs. We anticipate that CIPHER will inspire further exploration for the design of interactions within LLM agent systems, offering a new direction that could significantly influence future developments in the field.

==> table/llama1.tex <==
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\begin{table}[tb]

\centering
\caption{LLaMA-65B accuracy in percentage.}\label{table:llama1}

\resizebox{\textwidth}{!}{

\begin{tabular}{rlcccccc} 
\toprule
 Model & Method  & GSM8K & High School Math & Psychology & Formal Logic & Arithmetic & Biographies \\
\midrule
& Single Answer & 50.5 & 33.5 & 66.5  & 43.5 &  29.8 & -\\ 
 % \hline
 &  Major@5 & 57.8 & 36.7 &  67.0 & 44.4 & 31.0 & -\\ 
 % \hline
 &  Natural Language Debate  & 55.5 & 36.7 & 68.5 & 47.6  & 35.0  & -\\
&  CIPHER Debate (\textbf{ours}) & {\bf 58.8} & {\bf 38.5} & {\bf 70.5}  & {\bf 50.0} &\textbf{ 36.5 }& -\\
 \bottomrule
\end{tabular}
}

%%%% Note on the best pair of temperatures 
%% I/ Ours: 
%% - GSM8K (0.35, 0.8)  output_path 37/107 (trialID=15346825) 
%% - MMLU Formal logic (0.2, 0.85) output_path 10/32 (trialID=15509332) 
%% MMLU - Psychology  (0.08857, 0.3771) output_path 31/70 (trialID=15682661) 
%% MMLU - Math (0.48883089, 0.7969314)  output_path 58/68  (trialID=15633831)
%% Arithmetic (0.674, 1.426) , trialID 16997851

%% II/ Human
%% - GSM8K (0.1, 0.2) output_path 106/107  (trialID=15319218)
%% - MMLU Formal logic Temperatures=(0.2, 0.7) output_path 9/32 (trialID=15509329) 
%% MMLU - Psychology  (0.3, 0.4)  output_path 14/70  (trialID=15547543)
%% MMLU - Math  (0.4, 0.5) (trialID=15498378)  output_path 26/68
%% Arithmetic (0.013, 1.072)    trialID 16997853


\end{table}

==> table/llama1_vs_llama2_COMBINED_full.tex <==
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\begin{table}
% \vskip-0.1in
\caption{\textbf{Debate accuracies (\%) between LLaMA2-70B and LLaMA-65B} on \textbf{(a) Arithmetic} and \textbf{(b) GSM8K} datasets. We report the proportions of the changes in responses compared to the previous round in brackets. \textit{Agreement} indicates the consensus (\%) of the two debaters (i.e., they generate the same response). CIPHER debates result in higher accuracies in both debaters compared to NLD.} 
% \vskip-0.1in

\begin{subtable}{1\textwidth}
\sisetup{table-format=-1.2}   % 2 decimals, leave space for minus sign
\centering
\resizebox{\textwidth}{!}{
   \begin{tabular}{lccc|ccc}
\toprule
\multirow{2}{*}{\textbf{(a)} \textbf{Arithmetic}} & \multicolumn{3}{c|}{NLD~\citep{du2023improving}} & \multicolumn{3}{c}{CIPHER (ours)} \\
\cmidrule{2-4} \cmidrule{5-7}
& LLaMA2-70B & LLaMA-65B & Agreement & LLaMA2-70B & LLaMA-65B & Agreement \\
\midrule
Round 1 & 73.0 & 32.5 & 31.5 & 73.5 & 35.0 & 34.5\\
Round 2 & 69.0{\scriptsize(30.0)} & 56.0{\scriptsize(38.5)}  & 61.5 & 70.0{\scriptsize(27.0)} & 61.5{\scriptsize(40.0)} & 69.0\\
Round 3 & 72.0{\scriptsize(20.5)} & 60.5{\scriptsize(19.5)} & 77.5 & \textbf{74.5}{\scriptsize(13.5)} & \textbf{62.5}{\scriptsize(12.0)} & 78.0\\
\bottomrule
\end{tabular}
}
   % \caption{First subtable}
\label{tab:llama1_vs_llama2_arithmetic_full}
\end{subtable}

\begin{subtable}{1\textwidth}
\sisetup{table-format=4.0} % integer values only, up to 4 digits
\centering
\resizebox{\textwidth}{!}{
   \begin{tabular}{lccc|ccc}
\toprule
\multirow{2}{*}{\textbf{(b)} \textbf{ GSM8K }} \text{   }& \multicolumn{3}{c|}{NLD~\citep{du2023improving}} & \multicolumn{3}{c}{CIPHER (ours)} \\
\cmidrule{2-4} \cmidrule{5-7}
& LLaMA2-70B & LLaMA-65B & Agreement & LLaMA2-70B & LLaMA-65B & Agreement \\
\midrule
Round 1 & 61.0 & 51.3 & 51.5 & 61.5 & 48.0 & 44.0\\
Round 2 & 58.8{\scriptsize(32.5)} & 57.5{\scriptsize(27.3)} & 77.5 & 64.3{\scriptsize(24.5)} & 60.3{\scriptsize(39.5)} & 70.3\\
Round 3 & 61.8{\scriptsize(14.0)} & 59.0{\scriptsize(10.5)} & 88.8 & \textbf{64.8}{\scriptsize(16.8)} & \textbf{63.3}{\scriptsize(12.8)} & 83.8\\
\bottomrule

\end{tabular}
}
   % \caption{Second subtable}
   \label{tab:llama1_vs_llama2_gsm8k_full}
\end{subtable}
\vskip-0.1in


\label{tab:llama1_vs_llama2_full}
% \vskip-0.2in
\end{table}

==> table/llama1_vs_llama2_gsm8k_vector.tex <==
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\begin{table}[tb]

\centering
\caption{CIPHER (LLaMA2-70B \& LLaMA-65B) on GSM8K dataset.
}
\label{table:llama1_vs_llama2_gsm8k_vec}


\resizebox{\textwidth}{!}{

\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Debater} & \multirow{2}{*}{Round 1 Acc (\%)} & \multirow{2}{*}{Round 2 Acc (\%)} & \multirow{2}{*}{Round 3 Acc (\%)} & \multicolumn{3}{c}{Answer Change (\%)} \\
\cmidrule{5-7}
& & & & Round 1 $\rightarrow$ 2 & Round 2 $\rightarrow$ 3 & Round 1 $\rightarrow$ 3 \\
\midrule
LLaMA2-70B & 61.5        &   64.3  &         \textbf{64.8}  & 24.5 & 16.8 & 28.5\\
LLaMA-65B &   48.0   &        60.3      &    \textbf{63.3} & 39.5 & 12.8 & 41.3 \\
\midrule
Round Agreement & 44.0 & 70.3 & 83.8 &  &  &  \\
\bottomrule

\end{tabular}
}

\end{table}

%% log:output/log_2023-Sep-09/id17365166_2Llama-2-70b-hf_llama_65B_gsm8k_test_chau_full_seed63340_vec_nsols1_r3_temp0.35-0.65_nques400_2023-Sep-09--10-52-59.json



